Reward Machines for Cooperative Multi-Agent Reinforcement Learning

In cooperative multi-agent reinforcement learning, a collection of agents learns to interact in a shared environment to achieve a common goal. We propose the use of reward machines (RM) -- Mealy machines used as structured representations of reward functions -- to encode the team's task. The proposed novel interpretation of RMs in the multi-agent setting explicitly encodes required teammate interdependencies, allowing the team-level task to be decomposed into sub-tasks for individual agents. We define such a notion of RM decomposition and present algorithmically verifiable conditions guaranteeing that distributed completion of the sub-tasks leads to team behavior accomplishing the original task. This framework for task decomposition provides a natural approach to decentralized learning: agents may learn to accomplish their sub-tasks while observing only their local state and abstracted representations of their teammates. We accordingly propose a decentralized q-learning algorithm. Furthermore, in the case of undiscounted rewards, we use local value functions to derive lower and upper bounds for the global value function corresponding to the team task. Experimental results in three discrete settings exemplify the effectiveness of the proposed RM decomposition approach, which converges to a successful team policy an order of magnitude faster than a centralized learner and significantly outperforms hierarchical and independent q-learning approaches.

==> figures_flowcharts/decentralized_testing.tex <==

% We need layers to draw the block diagram
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\tikzset{auto, ->, >=stealth, node distance=2.2cm, every node/.style={scale=0.9, minimum size=0pt, inner sep=0pt}}

\def\blockOpacity{15}
\def\minBlockHeight{2em}

% Define a few styles and constants
\tikzstyle{qFunction}=[draw, fill=blue!\blockOpacity, text width=5em, 
    text centered, minimum height=\minBlockHeight]
    
\tikzstyle{rm}=[draw, fill=red!\blockOpacity, text width=3em, text centered, minimum height=\minBlockHeight]

\tikzstyle{comm}=[draw, fill=gray!\blockOpacity, text width=7em, text centered, minimum height=\minBlockHeight]

\tikzstyle{label}=[draw, fill=yellow!\blockOpacity, text width=2em, text centered, minimum height=\minBlockHeight]

\tikzstyle{envTransition}=[draw, fill=green!\blockOpacity, text width=5em, text centered, minimum height=\minBlockHeight]

\tikzstyle{agentDottedBox}=[fill=gray!5,rounded corners, draw=black!50, dashed]

\tikzstyle{envDottedBox}=[fill=green!5,rounded corners, draw=black!50, dashed]

\tikzstyle{branch}=[fill,shape=circle,minimum size=3pt,inner sep=0pt]

\def\blockdist{2.3}
\def\edgedist{2.5}

\def\verticalBlockDist{1.0}
\def\horizontalBlockDist{2.0}

\begin{tikzpicture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% AGENT 1
    \node (Q1) [qFunction] {\shortstack{Action\\selection}};
    \path (Q1.170)+(-1.5cm, 0.0cm) node (s1) {$s^1_{t}$};
    \path (Q1)+(-\horizontalBlockDist, -\verticalBlockDist) node (rm1) [rm] {$\RM_1$};
    \path (rm1)+(\horizontalBlockDist, 0.0) node (C1) [comm] {\shortstack{Team\\synchronization}};
    \path (C1)+(\horizontalBlockDist, 0.0) node (L1) [label] {$L_1$};
    
    % most paths between agent blocks
    \path [draw, ->] (s1) -- (Q1.170);
    \path [draw, ->] (L1) -- (C1);
    \path [draw, ->] (C1) -- (rm1.east); 
    \path [draw, ->] (rm1.north) |- node [near start, left=0.1cm] {$\RMCommonState^1_{t}$} (Q1.-170);
    
    % path between RM and L
    \path (rm1.north)+(0.0, 0.2) node [branch] (aboveRM1Hub) {};
    \path (L1.north)+(0.0, 0.2) node (aboveL1Hub) {};
    \path [draw, -] (aboveRM1Hub) -- (aboveL1Hub);
    \path [draw, ->] (aboveL1Hub) -- (L1.north);
    
    % Sync with teammates
    \path [draw, ->] (C1.-60) -- +(0.0, -0.5);
    \path [draw, <-] (C1.-120) -- +(0.0, -0.5);
    % \path (C1.south)+(0.6, -0.6) node {\shortstack{Team \\ sync}};
    
    \path (Q1)+(-1.5, -1.8) node (ellipsis) {$\mathbf{\vdots}$};
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% AGENT 2
    \path (Q1)+(0.0, -3.0) node (Q2) [qFunction] {\shortstack{Action\\selection}};
    \path (Q2.170)+(-1.5cm, 0.0cm) node (s2) {$s^\SGNumAgents_t$};
    \path (Q2)+(-\horizontalBlockDist, -\verticalBlockDist) node (rm2) [rm] {$\RM_\SGNumAgents$};
    \path (rm2)+(\horizontalBlockDist, 0.0) node (C2) [comm] {\shortstack{Team\\synchronization}};
    \path (C2)+(\horizontalBlockDist, 0.0) node (L2) [label] {$L_\SGNumAgents$};
    
    % most paths between agent blocks
    \path [draw, ->] (s2) -- (Q2.170);
    \path [draw, ->] (L2) -- (C2);
    \path [draw, ->] (C2) -- (rm2.east); 
    \path [draw, ->] (rm2.north) |- node [near start, left=0.1cm] {$\RMCommonState^\SGNumAgents_t$} (Q2.-170);
    
    % path between RM and L
    \path (rm2.north)+(0.0, 0.2) node [branch] (aboveRM2Hub) {};
    \path (L2.north)+(0.0, 0.2) node (aboveL2Hub) {};
    \path [draw, -] (aboveRM2Hub) -- (aboveL2Hub);
    \path [draw, ->] (aboveL2Hub) -- (L2.north);
    
    % Sync with teammates
    \path [draw, ->] (C2.-60) -- +(0.0, -0.5);
    \path [draw, <-] (C2.-120) -- +(0.0, -0.5);
    % \path (C2.south)+(0.6, -0.6) node {\shortstack{Team \\ sync}};
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ENVIRONMENT
    \path (Q1)+(4.3, 0.0) node (transition) [envTransition] {$\SGTransition(\cdot | \SGCommonJointState_t, \SGCommonJointAction_t)$};
    \path (transition)+(0.0, -1.5) node (L) [label] {$L$};
    \path (L)+(0.0, -1.5) node (rm) [rm] {$\RM$};
    
    \path [draw, ->] (transition.south) -- node [near start, right=0.1cm] {$\SGCommonJointState_{t+1}$} (L.north);
    \path [draw, ->] (L.south) -- node [right=0.1cm] {$\RMLabelingFunction(\SGCommonJointState_{t+1}, \RMCommonState_t)$} (rm.north);
    \path [draw, ->] (rm.south) -- +(0.0,-0.5) node [below=0.1cm] {\shortstack{Team task \\ reward}};
    
    \path (rm.west)+(-0.3, 0.0) node (rmStateHub1){};
    \path (rmStateHub1)+(0.0, 1.5) node (rmStateHub2){};
    
    \path [draw, -] (rm.west) -- (rmStateHub1);
    \path [draw, -] (rmStateHub1) -- node[right=0.1cm]{$\RMCommonState_t$} (rmStateHub2);
    \path [draw] (rmStateHub2) -- (L.west);
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ENV AGENT CONNECTIONS

    \def\radius{1mm}

    % Hubs/ branching points
    \path (transition)+(-1.4, 0.0) node [branch] (actionHub) {}; 
    \path (transition)+(0.0, -0.6) node [branch] (stateHub1) {};
    \path (stateHub1)+(-1.2, 0.0) node (stateHub2) {};
    \node (stateHub3) at (L1 -| stateHub2) [branch] {};
    \path (stateHub3 -| actionHub)+(-\radius, 0.0) node (arcHubLeft) {};
    \path (stateHub3 -| actionHub)+(\radius, 0.0) node (arcHubRight) {};

    % Action path
    \path [draw, -] (Q1.east) -- node [above] {$\SGCommonAction^1_t$} (actionHub);
    \path [draw, -] (Q2.east) -| node [near start, above] {$\SGCommonAction^\SGNumAgents_t$} (actionHub);
    \path [draw, ->] (actionHub) -- node [near start, above] {$\SGCommonJointAction_t$} (transition.west);

    % State return path
    \path [draw, -] (stateHub1) -- (stateHub2);
    \path [draw, ->] (stateHub2) |- node [near end, above] {$\SGCommonState^\SGNumAgents_{t+1}$} (L2.east);
    \path [draw, -] (stateHub3) -- (arcHubRight);
    \path [draw, ->] (arcHubLeft) -- node [above=0.1cm] {$\SGCommonState^1_{t+1}$} (L1.east);
    \draw [-] (arcHubRight) arc(0:180:\radius);

%%%%%%%%%%%%%%%%%%%%%%%%%%%% colored dotted areas
    \begin{pgfonlayer}{background}
        % Compute a few helper coordinates
        \path (Q1.west)+(-2.0,0.75) node (agent1_topLeft) {};
        \path (L1.east)+(+0.3,-0.5) node (agent1_bottomRight) {};
        \path[agentDottedBox](agent1_topLeft) rectangle (agent1_bottomRight);
        
        \path (Q2.west)+(-2.0,0.75) node (agent2_topLeft) {};
        \path (L2.east)+(+0.3,-0.5) node (agent2_bottomRight) {};
        \path[agentDottedBox](agent2_topLeft) rectangle (agent2_bottomRight);
        
        \path (transition)+(-1.0,0.75) node (env_topLeft) {};
        \path (rm)+(+1.0,-0.5) node (env_bottomRight) {};
        \path[envDottedBox](env_topLeft) rectangle (env_bottomRight);
    \end{pgfonlayer}
    
    % dotted box labels
    \path (agent1_topLeft)+(0.6, -0.25) node (agent1) {\ul{Agent 1}};
    \path (agent2_topLeft)+(0.6, -0.25) node (agent2) {\ul{Agent \SGNumAgents}};
    \path (env_topLeft)+(0.9, -0.25) node (env) {\ul{Environment}};

\end{tikzpicture}



==> figures_flowcharts/decentralized_training.tex <==

% We need layers to draw the block diagram
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\tikzset{auto, ->, >=stealth, node distance=2.2cm, every node/.style={scale=0.9, minimum size=0pt, inner sep=0pt}}

\def\blockOpacity{15}
\def\minBlockHeight{2em}

% Define a few styles and constants
\tikzstyle{qFunction}=[draw, fill=blue!\blockOpacity, text width=5em, 
    text centered, minimum height=\minBlockHeight]
    
\tikzstyle{rm}=[draw, fill=red!\blockOpacity, text width=3em, text centered, minimum height=\minBlockHeight]

\tikzstyle{comm}=[draw, fill=gray!\blockOpacity, text width=7em, text centered, minimum height=\minBlockHeight]

\tikzstyle{label}=[draw, fill=yellow!\blockOpacity, text width=2em, text centered, minimum height=\minBlockHeight]

\tikzstyle{envTransition}=[draw, fill=green!\blockOpacity, text width=5em, text centered, minimum height=\minBlockHeight]

\tikzstyle{agentDottedBox}=[fill=gray!5,rounded corners, draw=black!50, dashed]

\tikzstyle{envDottedBox}=[fill=green!5,rounded corners, draw=black!50, dashed]

\tikzstyle{branch}=[fill,shape=circle,minimum size=3pt,inner sep=0pt]

\def\blockdist{2.3}
\def\edgedist{2.5}

\def\verticalBlockDist{1.0}
\def\horizontalBlockDist{2.0}

\begin{tikzpicture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% AGENT i
    \node (Q1) [qFunction] {\shortstack{Action\\selection}};
    \path (Q1.170)+(-0.6cm, 0.0cm) node (s1) {$s^i_{t}$};
    \path (Q1)+(-\horizontalBlockDist, -\verticalBlockDist) node (rm1) [rm] {$\RM_i$};
    \path (rm1)+(\horizontalBlockDist, 0.0) node (C1) [comm] {\shortstack{Team\\synchronization}};
    \path (C1)+(\horizontalBlockDist, 0.0) node (L1) [label] {$L_i$};
    \path (Q1)+(0.0, \verticalBlockDist) node (QLearner) [qFunction]{Q-Learner};
    
    % most paths between agent blocks
    \path [draw, ->] (s1) -- (Q1.170);
    \path [draw, ->] (L1) -- (C1);
    \path [draw, ->] (C1) -- (rm1.east); 
    % \path [draw, ->] (rm1.45) |- node [near start, left=0.1cm] {$\RMCommonState^i_{t}$} (Q1.-170);
    \path [draw, ->] (QLearner.south) -- node [right, right=0.1cm] {$Q_i$ \textit{estimate}} (Q1.north);
    
    % path between RM and action selection
    \path (Q1.-170)+(-1.0, 0.0) node (leftOfActionSelection) [branch] {};
    \path [draw, ->] (leftOfActionSelection) -- (Q1.-170);
    
    % path between state and action selection
    \path (Q1.170)+(-0.3cm, 0.0cm) node (stateSplitter) [branch]{};
    \path [draw, ->] (stateSplitter) |- (QLearner.-165);
    
    % path between RM and L
    \path (rm1.45)+(0.0, 0.2) node [branch] (aboveRM1Hub) {};
    \path (L1.north)+(0.0, 0.2) node (aboveL1Hub) {};
    \path [draw, -] (aboveRM1Hub) -- (aboveL1Hub);
    \path [draw, ->] (aboveL1Hub) -- (L1.north);
    
    % path between RM and Q-learner
    \path [draw, ->] (rm1.45) |- (QLearner.180);
    \path [draw, ->] (rm1.135) |- (QLearner.165);
    \path (rm1.45)+(-0.2, 0.3) node {$\RMCommonState^i$};
    \path (rm1.135)+(-0.2, 0.3) node {$r$};
    
    
    % \path (C1.south)+(0.6, -0.6) node {\shortstack{Team \\ sync}};
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ENVIRONMENT
    \path (Q1)+(4.3, 0.0) node (transition) [envTransition] {$\SGTransition_i(\cdot | \SGCommonState_t^i, \SGCommonAction_t^i)$};
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ENV AGENT CONNECTIONS

    \def\radius{1mm}

    % Hubs/ branching points
    \path (transition)+(0.0, -\verticalBlockDist) node (stateHub1) {};

    % Action path
    \path (Q1.east)+(1.4, 0.0) node [branch] (rightOfActionSelection){};
    \path (rightOfActionSelection)+(0.3, 0.2) node {$\SGCommonAction^i_t$};
    \path [draw, -] (Q1.east) -- (rightOfActionSelection);
    \path [draw, ->] (rightOfActionSelection) -- (transition.west);
    \path [draw, ->] (rightOfActionSelection) |- (QLearner.-10);

    % State return path
    \path [draw, -] (transition.south) -- node [right, right=0.1cm]{$\SGCommonState^i_{t+1}$} (stateHub1);
    \path [draw, ->] (stateHub1) -- (L1.east);
    
    % State return path to Q Learner
    \path (transition.west)+(-0.6, -0.1) node (arcHubLower){};
    \path (transition.west)+(-0.6, 0.1) node (arcHubUpper){};
    \path (arcHubLower)+(0.0, -0.9) node [branch] (nextStateSplitter){};
    
    \draw [-] (arcHubLower) arc(-90:90:\radius);
    \path [draw, ->] (arcHubUpper) |- node [right, right=0.1cm] {$\SGCommonState_{t+1}^i$} (QLearner.10);
    \path [draw, -] (nextStateSplitter) -- (arcHubLower);
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%% team sync simulation block
    \path (C1)+(0.0, -\verticalBlockDist) node (simSync)[draw, fill=gray!\blockOpacity, text width=15em, text centered, minimum height=\minBlockHeight]{Simulated synchronization signal};
    
    % Sync with teammates
    \path [draw, ->] (C1.-60) -- (simSync.60);
    \path [draw, <-] (C1.-120) -- (simSync.120);

%%%%%%%%%%%%%%%%%%%%%%%%%%%% colored dotted areas
    \begin{pgfonlayer}{background}
        % Compute a few helper coordinates
        \path (Q1.west)+(-2.0,1.6) node (agent1_topLeft) {};
        \path (L1.east)+(+0.3,-0.5) node (agent1_bottomRight) {};
        \path[agentDottedBox](agent1_topLeft) rectangle (agent1_bottomRight);
        
        \path (transition)+(-1.0,0.75) node (env_topLeft) {};
        \path (transition)+(+1.0,-1.5) node (env_bottomRight) {};
        \path[envDottedBox](env_topLeft) rectangle (env_bottomRight);
    \end{pgfonlayer}
    
    % dotted box labels
    \path (agent1_topLeft)+(0.6, -0.25) node (agent1) {\ul{Agent $i$}};
    \path (env_topLeft)+(0.9, -0.25) node (env) {\ul{Environment}};

\end{tikzpicture}


